Federated Learning: Organizational Opportunities, Challenges, and Adoption Strategies

Restrictive rules for data sharing in many industries have led to the development of federated learning. Federated learning is a machine-learning technique that allows distributed clients to train models collaboratively without the need to share their respective training data with others. In this paper, we first explore the technical foundations of federated learning and its organizational opportunities. Second, we present a conceptual framework for the adoption of federated learning, mapping four types of organizations by their artificial intelligence capabilities and limits to data sharing. We then discuss why exemplary organizations in different contexts - including public authorities, financial service providers, manufacturing companies, as well as research and development consortia - might consider different approaches to federated learning. To conclude, we argue that federated learning presents organizational challenges with ample interdisciplinary opportunities for information systems researchers.

==> Figures/bise_research_agenda.tex <==

% to check: https://tex.stackexchange.com/questions/7208/how-to-vertically-center-the-text-of-the-cells

%\begin{landscape}

\begin{table}[h!]
\caption{A suggested research agenda for federated learning.}

\resizebox{\textwidth}{!}{%

\begin{tabular}{|m{.2\textwidth}|m{.8\textwidth}|}
\hline
\textbf{Research streams}                 & \textbf{Research questions}                                                                                                                 \\ \hline
\multirow{6}{*}{Technological}                & To what extent are \ac{FL} algorithms Byzantine Fault Tolerant?                                                                             \\ \cline{2-2} 
                                          & How can the central server assure trust among its clients?                                                                                  \\ \cline{2-2} 
                                          & How to train a fully decentralized \ac{FL} algorithm – that is without the need of a central server? What role can \ac{DLT} play?           \\ \cline{2-2} 
                                          & How to predict if a client decides to jeopardize the \ac{FL} model by adding false data?                                                    \\ \cline{2-2} 
                                          & What role does standardization of data preparation play in \ac{FL} systems?                                                                 \\ \cline{2-2} 
                                          & What is the critical mass level of data aggregation required for value creation in \ac{FL}?                                                 \\ \hline
\multirow{7}{\linewidth}{Organizational} & What organizational and collaborative settings establish the required trust for entities to partake in \ac{FL}?                             \\ \cline{2-2} 
                                          & How to implement \ac{FL} within an organization? To what extent can adoption be fostered?                                                   \\ \cline{2-2} 
                                          & What is the potential value of \ac{FL} to respective industries? How can the utility be valued?                                             \\ \cline{2-2} 
                                          & What business models allow to commercialize \ac{FL}? How to standardize \ac{FL} applications for collaboration and commercialization?       \\ \cline{2-2} 
                                          & How are decision rights and accountabilities enacted in a productive \ac{FL} setting?                                                       \\ \cline{2-2} 
                                          & What are necessary governance structures to balance self-interested parties from acting maliciously in a collaborative \ac{FL} environment? \\ \cline{2-2} 
                                          & How to establish governance frameworks in a inter-organizational setting? What are adequate organizational structures?                      \\ \hline
\multirow{5}{*}{Environmental}                   & What requirements are to be satisfied for \ac{FL} to function in a competitive environment?                                                 \\ \cline{2-2} 
                                          & How to avoid the establishment of oligopolies/cartels in a collaborative \ac{FL} setting?                                                   \\ \cline{2-2} 
                                          & What is the role of third parties in establishing trust for a \ac{FL}-based electronic marketplace?                                         \\ \cline{2-2} 
                                          & How to value individual contributions in a \ac{FL} environment? To what extent does it change dynamically?                                  \\ \cline{2-2} 
                                          & How to design a price model for a federated learning market? To what extent can existing pricing models be re-used/generalized?             \\
                                          \hline
\end{tabular}
 }
\label{tab:research_agenda}
\end{table}



%\end{landscape}

